Personalized Federated Learning with Server-Side Information

Personalized Federated Learning (FL) is an emerging research field in FL that learns an easily adaptable global model in the presence of data heterogeneity among clients. However, one of the main challenges for personalized FL is the heavy reliance on clients' computing resources to calculate higher-order gradients since client data is segregated from the server to ensure privacy. To resolve this, we focus on a problem setting where the server may possess its own data independent of clients' data -- a prevalent problem setting in various applications, yet relatively unexplored in existing literature. Specifically, we propose FedSIM, a new method for personalized FL that actively utilizes such server data to improve meta-gradient calculation in the server for increased personalization performance. Experimentally, we demonstrate through various benchmarks and ablations that FedSIM is superior to existing methods in terms of accuracy, more computationally efficient by calculating the full meta-gradients in the server, and converges up to 34.2% faster.

==> Sections/Methodology_.tex <==
\section{Federated Learning with Server Information Meta-Learning (Fed-SIM)}
\label{sec:method}


\subsection{\proposal: Problem Formulation}
In conventional FL, there are $n$ clients in a federated environment that tries to find a global model $\theta$ by optimizing the following problem:
\begin{equation}
\label{eq:fed_opt_problem}
\min_{\theta \in \mathbb{R}^d} f(\theta) := \frac{1}{n}\sum_{i=1}^n f_i(\theta)
\end{equation}

where $f_i: \mathbb{R}^d \rightarrow \mathbb{R}$ ($i = 1, ..., n$) denotes the expected loss over the data distribution of client $i$ such that 
\begin{equation}
\label{eq:loss}
f_i(\theta) = \mathbb{E}_{\mathcal{D}_i \sim p_i} [\tilde{f}_i (\theta; \mathcal{D}_i)]
\end{equation}
where $\mathcal{D}_i$ is a random data sample drawn from client $i$'s data distribution $p_i$ and $\tilde{f}_i(\theta; \mathcal{D}_i)$ is the loss corresponding with this data sample w.r.t. a global model $\theta$.


In contrast to Eq.(\ref{eq:fed_opt_problem}), we generate an \textit{adaptable} global model $\theta$ in a federated environment by formulating and solving a bi-level (server-side and client-side) problem defined as 
%
\begin{equation}
\label{eq: perfl_opt_problem_server}
\min_{\theta \in \mathbb{R}^d} F(\theta) := \frac{1}{n}\sum_{i=1}^n F_i(\theta)
\end{equation}
%
\begin{equation}
\label{eq: perfl_opt_problem_client}
F_i(\theta) = \min_{\phi_i \in \mathbb{R}^d} f_i'(\phi_i) := f_i(\phi_i) + \frac{\lambda}{2}||\phi_{i}-\theta||^2 
\end{equation}
%

where $\phi_i$  denotes the \textit{personalized model} of client $i$. Note that instead of the conventional loss in Eq. (\ref{eq:loss}), we define a different loss function $f_i'(\phi_i)$ that includes an $\ell_2$ regularization term where $\lambda$ is a scalar hyperparameter that denotes regularization strength.  
This custom loss is in accordance with ideas from \cite{li2020fedopt,moreau_envelopes} such that the personalized parameters $\phi_i$ are encouraged to tend towards the initial global parameters $\theta$, which improves convergence of the global model in non-i.i.d. data settings.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\textit{Fed-SIM}: Algorithm}
%
\textbf{Fed}erated Learning with \textbf{S}erver-Side \textbf{I}nformation \textbf{M}eta-Learning (\proposal) is a personalized FL  framework that aims to (\romannumeral 1) ensure client data privacy while (\romannumeral 2) producing high-quality meta gradients with (\romannumeral 3) minimal additional computation/communication overhead in clients compared to conventional FL.
%
In this section, we present the \proposal algorithm to solve for Eq. (\ref{eq: perfl_opt_problem}) in the context of Eq. (\ref{eq: perfl_opt_problem_client}).


In vanilla FL~\cite{mcmahan2017communicationefficient}, a centralized server generates a global model by averaging models from decentralized devices. At each round $t$, the server samples $S_t$ clients to optimize the global model $\theta_{t-1}$. 
Each client $i\in S_t$ updates $\theta_{t-1}$ with its private data $\mathcal{D}_i \sim p_i$ using gradient decent and uploads its optimized model $\phi_i$ back to the server. Finally, the server updates the global model to $\theta_t$ by averaging $\phi_i$ received from $S_t$. Note that $\mathcal{D}_i$ was never shared between the clients nor with the server.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Meta-Gradient Calculation}
\proposal follows the same principles as FL, but with additional computation for meta-gradients in the server to generate an easily adaptable global model.  We do this by optimizing $f'_i(\phi_i)$ in Eq.(\ref{eq: perfl_opt_problem_client}) such that 

\begin{equation}
\label{eq:lossgradients}
\nabla_{\phi_i} f'_i(\phi_i) = 0 \Rightarrow \nabla_{\phi_i} f_i(\phi_{i}) + \lambda(\phi_{i} - \theta)   = 0
\end{equation}
\begin{equation}
\label{eq:lossgradients_implicit}
\Rightarrow  \phi_i = \theta - \frac{1}{\lambda}\nabla_{\phi_i}f_i(\phi_i)
\end{equation}
which is an implicit equation that often arises in proximal point methods~\cite{imaml}. We can then differentiate and solve for $\frac{d\phi_i}{d\theta}$ in Eq.\ref{eq:lossgradients_implicit} (if we assume the derivative to exist) to acquire
\begin{equation}
\label{eq:metagradient}
\therefore \frac{d\phi_i}{d\theta} =\left(\textbf{I}+\frac{1}{\lambda} \nabla^2_{\phi_i} f_i(\phi_i)\right)^{-1}
\end{equation}
Thus, we can solve for Eq.(\ref{eq: perfl_opt_problem_server}) by optimizing $F_i(\theta)$ such that by the chain rule,
\begin{equation}
\label{eq:main}
\nabla_\theta F_i(\theta) = \frac{d\phi_i}{d\theta}\nabla_{\phi_i} f_i(\phi_i)
\end{equation}
\textbf{The main contribution of this work }comes from carefully leveraging the calculation of $\nabla_\theta F_i(\theta)$ \textit{between the clients and the server} such that we can calculate meta-gradients for multiple tasks without sharing data.

\begin{algorithm}[ht]
	\caption{\proposal: Client-Side}
    \label{algo:proposal_client}
\begin{algorithmic}
\REQUIRE{Step size $\alpha$, regularization strength $\lambda$, client data distribution $p_i$}
\FUNCTION {ClientUpdate$(i, \theta)$\textbf{:} // \textit{Run on client} $k$}
\STATE $\phi_{i, 0} \gets \theta$
\FOR{each local epoch $e$ from $1$ to $E$}
\STATE Sample a mini-batch $\mathcal{D}_i$ from distribution $p_i$
\STATE $\phi_{i, e} \gets \phi_{i, e-1} - \alpha \nabla_{\phi} \tilde{f}_i' (\phi_{i, e-1}; \mathcal{D}_i)$
\ENDFOR
\STATE Return $\phi_{i, E}$ to server
\ENDFUNCTION
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Client-side algorithm} 
%
The client's main purpose is to generate a personalized model $\phi_i^*$ which is a $\gamma_i$-approximation of $\phi_i$  that satisfies  

\begin{equation}
\label{eq:perfed_meta_gradients}
\mathbb{E}\left [||\phi_i^* - \phi_i|| \right] \leq \gamma_i
\end{equation}
%
In practice, $\gamma_i$ is often set to a constant number~\cite{moreau_envelopes,li2020fedopt} such that $\phi_i^*$ can be obtained by calculating local gradient updates $\phi_{i,e} \leftarrow \phi_{i,e-1} - \nabla_\phi f_i'(\phi_{i,e-1})$ for $E$ epochs such that $\phi_{i,E}$ satisfies Eq.(\ref{eq:perfed_meta_gradients}).
To calculate $\nabla_\phi f_i'(\phi_{i,e-1})$ in practice, we use an unbiased estimate $\nabla_{\phi} \tilde{f}_i'(\phi_{i,e-1}; \mathcal{D}_i)$ by sampling a mini-batch of data $\mathcal{D}_i$ from distribution $p_i$. This process is illustrated in algorithm \ref{algo:proposal_client}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[ht]
    \caption{\proposal: Server-Side}
    \label{algo:proposal_server}
\begin{algorithmic}
    \REQUIRE{Step size $\beta$, $\delta$, server data distribution $p_s$}
    \STATE Initialize $\theta_0$
    \FOR{each round $t=1,2,...$}
    	\STATE Sample a mini-batch  $\mathcal{D}_s$ from distribution $p_s$
    	\STATE $S_t \gets $ Random sample of $m$ clients ($1 \le m \le N$)
    	\FOR{each client $i \in S_t$ \textbf{in parallel}}
        		\STATE $\phi_i \gets$ ClientUpdate($i$, $\theta_{t-1}$) (Algorithm~\ref{algo:proposal_client})
        		\STATE Calculate $v_i = \nabla_\phi f_i(\phi_i)$ with Eq.\eqref{eq:reptile}
        		\STATE Calculate $d_i = \nabla^2_\phi f_i(\phi_i)v_i$ using $\mathcal{D}_s$ with Eq.\eqref{eq:secondorderhessian}
        		\STATE Calculate meta-gradient $\nabla_\theta F_i (\theta_{t-1}) = v_i - \delta d_i$
       	 		\STATE Update $\tilde{\phi}_i \gets \phi_i - \beta \nabla_\theta F_i (\theta_{t-1})$
    	\ENDFOR
   	 	\STATE $\theta_{t} \gets \frac{1}{m}\sum_{i \in S_t}\tilde{\phi}_i$
    \ENDFOR
\end{algorithmic}
\end{algorithm}


\textbf{Server-side algorithm} 
%
The server's main goal is to solve for Eq.(\ref{eq: perfl_opt_problem_server}) by optimizing Eq.(\ref{eq:main}) by using $\phi_i$ received by the clients. In each round $t$, the central server (\romannumeral 1) samples $m$ clients, (\romannumeral 2) calculates meta-gradients $\nabla_\theta F_i(\theta_{t-1})$ for each of these clients using local model $\phi_i$ and server data $\mathcal{D}_s$ and (\romannumeral 3) updates the global model from $\theta_{t-1}$ to $\theta_t$ using these meta-gradients.  

Note that from Eq.(\ref{eq:metagradient}), $\nabla_\theta F_i(\theta_{t-1})$ is no longer dependent on the original meta model $\theta_{t-1}$, while corresponding with the personalized model $\phi_i$. Since the meta-gradient $\nabla_\theta F_i(\theta_{t-1})$ is decoupled from $\theta_{t-1}$, the server is able to approximate the meta-gradient without needing an entire history of client $i$'s local updates. This is why unlike \texttt{Per-FedAvg}, which only updates the local model with one inner loop, \proposal can allow clients to utilize multi-step gradient decent for local optimization. 

We can see from Eq.(\ref{eq:main}) that the calculation of $\nabla_\theta F_i(\theta_{t-1})$ requires two terms: 
%
\vspace{-1ex}
\begin{enumerate}
\item A first-order gradient $v_i = \nabla_\phi f_i(\phi_i)$
\item A Hessian-vector product $d_i = \nabla^2_\phi f(\phi_i) v_i$
\end{enumerate}
\vspace{-1ex}
%
Unlike previous meta-learning approaches for personalized FL, \textbf{we propose to calculate} \textbf{both} $v_i$ and $d_i$ \textbf{using the server}, without requiring additional information from clients.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{First-order gradient} 
%
As in Per-\texttt{FedAvg}, the first-order meta-gradient $v_i$ ideally requires a client-specific query dataset $\mathcal{D}_i^q$ to calculate an unbiased estimate $\nabla_{\phi} \tilde{f}_i (\phi_i;\mathcal{D}_i^q)$.
%
However, in \proposal, since the server does not have the required client data, we instead approximate $v_i$ by using the weight difference between a personalized model $\phi_i$ and global model  $\theta$ such that 
%
\begin{equation}
\label{eq:reptile}
    v_i = \nabla_{\phi} f_i (\phi_i)\approx \theta - \phi_i
\end{equation}
%
The intuition behind this method comes from the assumption that the derivative of $\nabla_\phi f'_i(\phi_i)$ in Eq.(\ref{eq:lossgradients}) at a stationary point $\phi_i$ becomes negligibly small. 

A possible alternative to calculate $v_i$ at the server is to sample a query dataset $\mathcal{D}^q_s$ from server data distribution $p_s$ and calculate $\nabla_\phi \tilde{f}_i(\phi_i; \mathcal{D}^q_s)$.  A limitation to this approach comes from the fact that $\mathcal{D}^q_s$ does not come from the data distribution of client $i$. Our ablation study in Section~\ref{sec:eval} will show that the weight difference approximation is superior to direct calculation using server data.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Second-order meta gradient
\textbf{Second-order meta-gradient} 
%
To calculate $d_i$, instead of separately computing the Hessian $\nabla^2_{\phi} f_i(\phi_i)$, we approximate the entire Hessian-vector product $d_i$ by using Hessian-free estimation~\cite{convergencetheorymaml} as follows: 
%
\begin{eqnarray}
\label{eq:secondorderhessian}
    d_i &=& \nabla^2_\phi f_i(\phi_i) v_i  \nonumber \\
    &\approx& \frac{\nabla_\phi f_i(\phi_i+\delta v_i)-\nabla_\phi f_i(\phi_i-\delta v_i)}{2\delta}
\end{eqnarray}
%
This approximation produces an error of at most $\rho \delta \|v_i\|^2$, where $\rho$ is the parameter for Lipschitz continuity of the Hessian of $f$. 


Ideally, calculating unbiased estimates for the two first-order gradients $\nabla_\phi f_i(\phi_i+\delta v_i)$ and $\nabla_\phi f_i(\phi_i-\delta v_i)$ in Eq.(\ref{eq:secondorderhessian})  requires additional client-specific data $\mathcal{D}_s^h \sim p_i$. 
%
We take an alternative approach since the server does not have client data. The server samples $\mathcal{D}_s$ from its own data distribution $p_s$ and calculates  $\nabla_\phi \tilde{f}_i(\phi_i+\delta v_i; \mathcal{D}_s)$ and $\nabla_\phi \tilde{f}_i(\phi_i-\delta v_i; \mathcal{D}_s)$. 


Note that we reuse the same dataset $\mathcal{D}_s$ to calculate $d_i$ for all clients in $S_t$. Given that the server data distribution $p_s$ is likely to be different from each client's data distribution $p_i$, the quality of $d_i$ calculated using $\mathcal{D}_s$ may not be ideal. 
%
Nevertheless, we hypothesized that using the non-ideal second-order terms would improve performance over disregarding the second-order terms altogether. The effectiveness of this approximation will be  empirically evaluated in Sections~\ref{sec:eval} and \ref{sec:stat}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\textit{Fed-SIM}: Design Choices}
%
Overall, the key design choices for the \proposal framework can be summarized as follows:
%
\vspace{-1ex}
\begin{itemize}[leftmargin=*]
    \item \textbf{Custom loss for local optimization}: Each client adds an $\ell_2$ regularization term to its loss function as in Eq.\eqref{eq: perfl_opt_problem_client} when optimizing a global model locally. This decouples meta gradient calculation (at the server) from local optimization history (at the clients).
    %
    \item \textbf{First-order meta gradient calculation using weight differences}: Despite the existence of server data, the server calculates the first-order gradient $v_i$ using (client-specific) weight differences as in Eq.\eqref{eq:reptile} instead of using the server data. %With our custom loss, the former is not only easier to calculate, but also mathematically more accurate than the latter.
    %
    \item \textbf{Second-order meta gradient calculation using server data}: The server calculates second-order gradient $d_i$ in a Hessian-Free way as in Eq.\eqref{eq:secondorderhessian}. This approximation requires two terms, which are calculated using server data $\mathcal{D}_s \sim p_s$ as $\nabla_\phi f_i(\phi_i+\delta v_i; \mathcal{D}_s)$ and $\nabla_\phi f_i(\phi_i-\delta v_i; \mathcal{D}_s)$. 
\end{itemize}
\vspace{-1ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\vspace{-2ex}
\caption{Non-i.i.d. datasets and model architectures for federated learning benchmark~\cite{chaoyanghe2020fedml}.}
\label{table:datasets}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccc}
\hline
\multirow{2}{*}{\textbf{Datasets}} & \textbf{\# of training} & \textbf{Non-i.i.d.} & \textbf{\# of partitions} & \textbf{\# of partitions} & \textbf{Baseline} \\
 & \textbf{samples} & \textbf{partition method} & \textbf{for clients} & \textbf{reserved server data} & \textbf{model architecture} \\ \hline\hline
Federated EMNIST & 671585 & realistic & 3230 & 0$-$170 & CNN (2 Conv + 2 FC) \\
CIFAR-100        & 50000  & Pachinko & 475  & 0$-$25 & ResNet-18 + group normalization \\
Shakespeare      & 16068  & realistic & 680  & 0$-$35 & RNN (2 LSTM + 1 FC) \\
StackOverflow    & 135818730 & realistic & 325354 & 0$-$17123 & RNN (1 LSTM + 2 FC) \\\hline
\end{tabular}}
\vspace{-2ex}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htbp]
    \includegraphics[width=\linewidth]{Graphs/Accuracy_Server.png}
    \vspace{-4ex}
    \caption{Effect of the proportion of server data on method performance when $E=5$.}
    \vspace{-2ex}
    \label{fig:acc_server}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With these design choices, \proposal ensures that data remains on the client while also ensuring that the calculation and communication done on the client is no more intensive than that done during standard federated learning (\texttt{FedAvg} or FedProx). 

